Evaluating Organization Security: User Stories of European Union NIS2 Directive

The NIS2 directive requires EU Member States to ensure a consistently high level of cybersecurity by setting risk-management measures for essential and important entities. Evaluations are necessary to assess whether the required security level is met. This involves understanding the needs and goals of different personas defined by NIS2, who benefit from evaluation results. In this paper, we consider how NIS2 user stories support the evaluation of the level of information security in organizations. Using requirements elicitation principles, we extracted the legal requirements from NIS2 from our narrowed scope, identified six key personas and their goals, formulated user stories based on the gathered information, and validated the usability and relevance of the user stories with security evaluation instruments or methods we found from the literature. The defined user stories help to adjust existing instruments and methods of assessing the security level to comply with NIS2. On the other hand, user stories enable us to see the patterns related to security evaluation when developing new NIS2-compliant security evaluation methods to optimize the administrative burden of entities.

==> NIS2Articles.tex <==
Article 18 (1) requires ENISA to compile the Report on the state of cybersecurity in the Union
ENISA shall adopt, in cooperation with the Commission and the Cooperation Group, a biennial report on the state of cybersecurity in the Union and shall submit and present that report to the European Parliament. The report shall, inter alia, be made available in machine-readable data and include the following: (b) an assessment of the development of cybersecurity capabilities in the public and private sectors across the Union; (c) an assessment of the general level of cybersecurity awareness and cyber hygiene among citizens and entities, including small and medium-sized enterprises; (e) an aggregated assessment of the level of maturity of cybersecurity capabilities and resources across the Union, including those at sector level, as well as of the extent to which the Member States’ national cybersecurity strategies are aligned.''

Art 19(1.a) The peer reviews shall cover at least one of the following: a) the level of implementation of the cybersecurity risk-management measures /---/ %and reporting obligations 
   laid down in Articles 21 %and 23
   ; 
   
Art 20 (1) Member States shall ensure that the management bodies of essential and important entities approve the cybersecurity risk-management measures taken by those entities in order to comply with Article 21, oversee its implementation and can be held liable for infringements by the entities of that Article.

Art 20(2)Member States shall ensure that the members of the management bodies of essential and important entities are required to follow training, and shall encourage essential and important entities to offer similar training to their employees on a regular basis, in order that they gain sufficient knowledge and skills to enable them to identify risks and assess cybersecurity risk-management practices and their impact on the services provided by the entity.
   
Art 21 (2) 2.  
    The measures referred to in paragraph 1 shall be based on an all-hazards approach that aims to protect network and information systems and the physical environment of those systems from incidents, and shall include at least the following:
	a) policies on risk analysis and information system security;
	b) incident handling;
	c) business continuity, such as backup management and disaster recovery, and crisis management;
	d) supply chain security, including security-related aspects concerning the relationships between each entity and its direct suppliers or service providers;
	e) security in network and information systems acquisition, development and maintenance, including vulnerability handling and disclosure;
	f) policies and procedures to assess the effectiveness of cybersecurity risk-management measures;
	g) basic cyber hygiene practices and cybersecurity training;
	h) policies and procedures regarding the use of cryptography and, where appropriate, encryption;
	i) human resources security, access control policies and asset management;
	j) the use of multi-factor authentication or continuous authentication solutions, secured voice, video and text communications and secured emergency communication systems within the entity, where appropriate.

Art 21 (3.)  Member States shall ensure that, when considering which measures referred to in paragraph 2, point (d), of this Article are appropriate, entities take into account the vulnerabilities specific to each direct supplier and service provider and the overall quality of products and cybersecurity practices of their suppliers and service providers, including their secure development procedures.


Art 21(4) Member States shall ensure that an entity that finds that it does not comply with the measures provided for in paragraph 2 takes, without undue delay, all necessary, appropriate and proportionate corrective measures.

Art 31 General aspects concerning supervision and enforcement
2.  Member States may allow their competent authorities to prioritise supervisory tasks. Such prioritisation shall be based on a risk-based approach. To that end, when exercising their supervisory tasks provided for in Articles 32 and 33, the competent authorities may establish supervisory methodologies allowing for a prioritisation of such tasks following a risk-based approach.

Art32(2) a)  on-site inspections and off-site supervision, including random checks conducted by trained professionals;
e) requests for information necessary to assess the cybersecurity risk-management measures adopted by the entity concerned, including documented cybersecurity policies, as well as compliance with the obligation to submit information to the competent authorities pursuant to Article 27;

Art32(4)  Member States shall ensure that their competent authorities, when exercising their enforcement powers in relation to essential entities, have the power at least to: d) order the entities concerned to ensure that their cybersecurity risk-management measures comply with Article 21 or to fulfil the reporting obligations laid down in Article 23, in a specified manner and within a specified period;
f) order the entities concerned to implement the recommendations provided as a result of a security audit within a reasonable deadline;
g) designate a monitoring officer with well-defined tasks for a determined period of time to oversee the compliance of the entities concerned with Articles 21 and 23;

Art 33(2) Member States shall ensure that the competent authorities, when exercising their supervisory tasks in relation to important entities, have the power to subject those entities at least to: a) on-site inspections and off-site ex post supervision conducted by trained professionals.


PERSONAS goals:
%===============================
\subsection{Member State (state-level decision maker)} 
Member States' goal is to ensure the effective implementation and oversight of cybersecurity risk-management measures by essential and important entities. This requires assessing and improving the level of compliance with Articles 20 and 21, including the approval and accountability of management bodies for these risk-management measures mentioned in Art 20. To achieve this goal, Member States should evaluate the entity's cybersecurity level based on an all-hazards approach covering cybersecurity policies and practices such as risk analysis, incident handling, business continuity, supply chain security, network, basic cyber hygiene and training practices, human resources security and the use of encryption, among others. 
Additionally, since the goal of the Member State is to ensure a commonly high level of cybersecurity (Art 1), in cases of deviations, they must allocate resources towards addressing and correcting vulnerabilities once identified.

Art 1 (1)
Art 19(1.a) 
Art 20 (1) 
Art 21 (2) 2.  
Art 21 (4) 
%===============================
\subsection{Supervisory Authority} 
The goal of the Member State supervisory authority is to ensure effective risk-based supervision, compliance, and enforcement of regulatory requirements related to cybersecurity risk management. Specifically, the authority aims to evaluate organizational compliance with Articles 21, particularly the implementation of cybersecurity risk-management measures;
prioritize supervisory tasks, aligning with the risk-based approach (Article 31); 
identify entities where entities do not comply with the regulatory requirements and ensure they take prompt, necessary, and proportionate corrective measures (Article 21(4));
support off-site supervision (Article 32), facilitating inspections to verify the effectiveness of cybersecurity measures and risk management;
ensure that entities implement the recommendations from security audits within reasonable deadlines (Article 32(4)(f)), thus improving their overall cybersecurity posture.
By obtaining security measurement results, the supervisory authority can better monitor and enforce cybersecurity regulations, ensuring that organizations mitigate risks in compliance with national and EU-level cybersecurity frameworks. Prioritising helps supervisory authorities focus resources on higher-risk organizations or areas where non-compliance or vulnerabilities are more likely and more damaging.

Art21(4) 
Art31(2)
Art32(2)
Art32(4)
Art33(2)


%===============================
\subsection{ENISA}
ENISA's goal in Member States is to collect and assess data on cybersecurity capabilities, awareness, and hygiene levels across the Union. Through this, ENISA aims to assess the development of cybersecurity capabilities in the public and private sectors (Article 18(1)(b));
assess the general level of cybersecurity awareness and cyber hygiene among citizens and entities, including small and medium-sized enterprises (Article 18(1)(c)), and 
provide an aggregated assessment of the maturity level of cybersecurity capabilities and resources across the European Union, including at the sector level, and evaluate the alignment of national cybersecurity strategies of Member States (Article 18(1)(e)).
The collected data will enable ENISA to produce reliable reports and make recommendations on improving cybersecurity in the Union and strengthening the capabilities of the Member States.

Art18(1)


%===============================
\subsection{External Security Consultant} % sõltumatu hinnang organisatsiooni hetkeolukorrale (erinevad eesmärgid - olukorra teadlikkus)
The goal of the external consultant is to get a quick overview of the institution's cyber security to plan the institution's consulting activities that would ensure compliance with NIS2 requirements (Art 20(2), Art 21 (2)). Such external consultants can be hired by the entity or be the institutions advising specific entities at the national level to increase the cybersecurity level of the specific domain entities.

Art20(2)
Art21(2) 

%===============================
\subsection{Members of the Management Bodies}
The goal of the management body of the entity is to ensure comprehensive oversight and risk management through enhancing awareness and competence to identify risks and evaluate cybersecurity risk-management practices effectively, in compliance with Article 20(2); ensuring that the entity adopts a comprehensive, all-hazards approach to protecting network and information systems (Article 21(2), and strengthens its ability to handle cybersecurity risks effectively, thus protecting its services and maintaining operational resilience over time (Article 21(2).

Art20(2)
Art21(2)

%===============================
\subsection{Entities as a Partner of Supplier and Service Provider }
The goal of the entity, as outlined in Articles 21(2)(d) and 21(3), is to protect its network and information systems by addressing supply chain security risks. This includes evaluating the specific vulnerabilities of each supplier and service provider, ensuring they meet high cybersecurity standards, and considering the overall quality of their products and secure development practices.

Art21(2)
Art21(3) 
%===============================
%===============================



==> drafts.tex <==
%NIS2 clauslid tabelkujul

\begin{longtable}{|p{0.55in}|p{3.0in}|p{1.1in}|}

\caption{NIS2 clauses related with security evaluation of entities. All crosscheck keywords are marked in italic}
\label{tab:clauses}\\
%\begin{tabular}
\hline
NIS2 Article and paragraph No &  Quote & Notes\\
\hline

Art1(1)
& This Directive lays down \textit{measure}s that aim to achieve a high common \textit{level} of cybersecurity across the Union, with a view to improving the functioning of the internal market.
& \\
\hline


Art18(1) 
&  requires \underline{ENISA} \textbf{to compile the Report on the state of cybersecurity} in the Union
ENISA \textbf{shall adopt}, in cooperation with the Commission and the Cooperation Group, a biennial \textit{report on the state of cybersecurity} in the Union and \textbf{shall submit and present} that report to the \underline{European Parliament}. The report \textbf{shall}, inter alia, be made available in machine-readable data and \textbf{include the following}: (b) an \textbf{assessment of the development of cybersecurity capabilities in \underline{the public and private sectors}} across the Union; (c) \textbf{an assessment of the general level of cybersecurity awareness and cyber hygiene} among citizens and \underline{entities, including small and medium-sized enterprises}; (e) an aggregated \textbf{assessment of the level of maturity} of cybersecurity capabilities and resources across the Union, including those at sector level, as well as of the extent to which the Member States’ national cybersecurity strategies are aligned.
& Persona: ENISA 

\\
\hline

Art19(1) 
&  The \underline{peer reviews} \textbf{shall cover} at least one of the following: a) the \textbf{level of implementation of the cybersecurity risk-management measures} /---/ %and reporting obligations 
   laid down in Articles 21 %and 23 
& MS peer reviews\\
\hline

Art20(1) 
& \underline{Member States} shall \textbf{ensure that the \underline{management bodies of essential and important entities} approve the cybersecurity risk-management \textit{measure}s taken} by those entities in order to comply with Article 21, \textbf{oversee its implementation} and can be held liable for infringements by the entities of that Article. 
& MS oversee\\
\hline

Art20(2)
& \underline{Member States} \textbf{shall ensure} that the \underline{members of the management bodies of essential and important entities} are required to follow training, and shall encourage essential and important entities to offer similar training to their \underline{employees} on a regular basis, in order that they gain sufficient knowledge and skills to enable them to identify risks and \textit{assess cybersecurity risk-management practices} and their impact on the services provided by the entity.
& MS ensures supplier assessing\\
\hline

Art21(1)
&\underline{Member States} \textbf{shall ensure} that \textbf{\underline{essential and important entities} take appropriate and proportionate technical, operational and organizational measures to manage the risks} posed to the security of network and information systems which those entities use for their operations or for the provision of their services, and to prevent or minimise the impact of incidents on recipients of their services and on other services.

&
\\
\hline

Art21(2)     
& The \textit{measure}s referred to in paragraph 1 \textbf{shall be based on an all-hazards approach} that aims to protect \underline{network and information systems and the physical environment of those systems} from incidents, and shall include at least the following:
	a) policies on risk analysis and information system security;
	b) incident handling;
	c) business continuity, such as backup management and disaster recovery, and crisis management;
	d) supply chain security, including security-related aspects concerning the relationships between each entity and its direct suppliers or service providers;
	e) security in network and information systems acquisition, development and maintenance, including vulnerability handling and disclosure;
	f) policies and procedures to assess the effectiveness of cybersecurity risk-management \textit{measure}s;
	g) basic cyber hygiene practices and cybersecurity training;
	h) policies and procedures regarding the use of cryptography and, where appropriate, encryption;
	i) human resources security, access control policies and asset management;
	j) the use of multi-factor authentication or continuous authentication solutions, secured voice, video and text communications and secured emergency communication systems within the entity, where appropriate. 
& MS ensures entities all-hazard approach\\
\hline

Art21(3)  
& \underline{Member States} shall \textbf{ensure} that, when considering which measures referred to in paragraph 2, point (d), of this Article are appropriate, \underline{entities} \textit{take into account the vulnerabilities} specific to each direct \underline{supplier and service provider} and the overall quality of products and \textit{cybersecurity practices of their suppliers and service providers}, including their secure development procedures.
& MS ensures entities' supplier and service provider vulnerabilities evaluation\\
\hline


Art21(4) 
& \underline{Member States} shall \textit{ensure} that \underline{an entity} that finds that it does not comply with the measures provided for in paragraph 2 \textit{takes}, without undue delay, \textit{all necessary, appropriate and proportionate corrective measures}.
& MS ensures entities improvements\\
\hline


Art31(2) 
& \underline{Member States}\textbf{ may allow their \underline{competent authorities} to prioritise supervisory tasks}. Such prioritisation s\textbf{hall be based on a risk-based approach}. To that end, when exercising their supervisory tasks provided for in Articles 32 and 33, the \underline{competent authorities} may establish supervisory methodologies allowing for a prioritisation of such tasks following a risk-based approach.
& Supervisory tasks prioritisation\\
\hline


Art32(2) 
 \underline{Member States} \textbf{shall ensure} that \underline{the competent authorities}, when exercising their supervisory tasks in relation to \underline{essential entities}, have the power to subject those entities at least to:
& a)  on-site inspections and \textit{off-site supervision}, including random checks conducted by trained professionals;
e) r\textit{equests for information necessary to \textit{assess} the cybersecurity risk-management measures} adopted by \underline{the entity} concerned, including documented cybersecurity policies, as well as compliance with the obligation to submit information to the \underline{competent authorities} pursuant to Article 27;
& Supervisory off-site assessment \\
\hline


Art32(4)  
& \underline{Member States} \textbf{shall ensure} that their \underline{competent authorities}, when exercising their enforcement powers in relation to essential entities, have the power at least to: d) order the \underline{entities} concerned to \textit{ensure} that their cybersecurity risk-management \textit{measure}s comply with Article 21 /.../ %or to fulfil the reporting obligations laid down in Article 23
, in a specified manner and within a specified period;
f) order the \underline{entities} concerned to implement the recommendations provided as a result of a security audit within a reasonable deadline;
g) designate a monitoring officer with well-defined tasks \textbf{for a determined period of time to oversee the compliance} of the \underline{entities} concerned with Articles 21 /.../%and Article 23;
&  Supervisory oversee\\
\hline


Art33(2) 
& \underline{Member States} \textbf{shall ensure} that \underline{the competent authorities}, when exercising their supervisory tasks in relation to \underline{important entities}, have the power to subject those entities at least to: a) \textit{on-site inspections and off-site ex post supervision} conducted by \underline{trained professionals}.
& Ex post off-site supervision \\
\hline

%\end{tabular}
\end{longtable}

%NIS2 nõuded textina:
Art1(1)\\
This Directive lays down \textit{measure}s that aim to achieve a high common \textit{level} of cybersecurity across the Union, with a view to improving the functioning of the internal market.


Art18(1) \\
requires \underline{ENISA} \textbf{to compile the Report on the state of cybersecurity} in the Union
ENISA \textbf{shall adopt}, in cooperation with the Commission and the Cooperation Group, a biennial \textit{report on the state of cybersecurity} in the Union and \textbf{shall submit and present} that report to the \underline{European Parliament}. The report \textbf{shall}, inter alia, be made available in machine-readable data and \textbf{include the following}: (b) an \textbf{assessment of the development of cybersecurity capabilities in \underline{the public and private sectors}} across the Union; (c) \textbf{an assessment of the general level of cybersecurity awareness and cyber hygiene} among citizens and \underline{entities, including small and medium-sized enterprises}; (e) an aggregated \textbf{assessment of the level of maturity} of cybersecurity capabilities and resources across the Union, including those at sector level, as well as of the extent to which the Member States’ national cybersecurity strategies are aligned.


Art19(1)\\ 
The \underline{peer reviews} \textbf{shall cover} at least one of the following: a) the \textbf{level of implementation of the cybersecurity risk-management measures} /---/ %and reporting obligations 
   laid down in Articles 21 %and 23 


Art20(1) \\
\underline{Member States} shall \textbf{ensure that the \underline{management bodies of essential and important entities} approve the cybersecurity risk-management \textit{measure}s taken} by those entities in order to comply with Article 21, \textbf{oversee its implementation} and can be held liable for infringements by the entities of that Article. 

Art20(2)\\
\underline{Member States} \textbf{shall ensure} that the \underline{members of the management bodies of essential and important entities} are required to follow training, and shall encourage essential and important entities to offer similar training to their \underline{employees} on a regular basis, in order that they gain sufficient knowledge and skills to enable them to identify risks and \textit{assess cybersecurity risk-management practices} and their impact on the services provided by the entity.


Art21(1)\\
\underline{Member States} \textbf{shall ensure} that \textbf{\underline{essential and important entities} take appropriate and proportionate technical, operational and organizational measures to manage the risks} posed to the security of network and information systems which those entities use for their operations or for the provision of their services, and to prevent or minimise the impact of incidents on recipients of their services and on other services.

Art21(2) \\    
The \textit{measure}s referred to in paragraph 1 \textbf{shall be based on an all-hazards approach} that aims to protect \underline{network and information systems and the physical environment of those systems} from incidents, and shall include at least the following:
	a) policies on risk analysis and information system security;
	b) incident handling;
	c) business continuity, such as backup management and disaster recovery, and crisis management;
	d) supply chain security, including security-related aspects concerning the relationships between each entity and its direct suppliers or service providers;
	e) security in network and information systems acquisition, development and maintenance, including vulnerability handling and disclosure;
	f) policies and procedures to assess the effectiveness of cybersecurity risk-management \textit{measure}s;
	g) basic cyber hygiene practices and cybersecurity training;
	h) policies and procedures regarding the use of cryptography and, where appropriate, encryption;
	i) human resources security, access control policies and asset management;
	j) the use of multi-factor authentication or continuous authentication solutions, secured voice, video and text communications and secured emergency communication systems within the entity, where appropriate. 

Art21(3) \\ 
\underline{Member States} shall \textbf{ensure} that, when considering which measures referred to in paragraph 2, point (d), of this Article are appropriate, \underline{entities} \textit{take into account the vulnerabilities} specific to each direct \underline{supplier and service provider} and the overall quality of products and \textit{cybersecurity practices of their suppliers and service providers}, including their secure development procedures.


Art21(4) \\
\underline{Member States} shall \textit{ensure} that \underline{an entity} that finds that it does not comply with the measures provided for in paragraph 2 \textit{takes}, without undue delay, \textit{all necessary, appropriate and proportionate corrective measures}.

Art31(2) \\
\underline{Member States}\textbf{ may allow their \underline{competent authorities} to prioritise supervisory tasks}. Such prioritisation s\textbf{hall be based on a risk-based approach}. To that end, when exercising their supervisory tasks provided for in Articles 32 and 33, the \underline{competent authorities} may establish supervisory methodologies allowing for a prioritisation of such tasks following a risk-based approach.

Art32(2) 
 \underline{Member States} \textbf{shall ensure} that \underline{the competent authorities}, when exercising their supervisory tasks in relation to \underline{essential entities}, have the power to subject those entities at least to:
a)  on-site inspections and \textit{off-site supervision}, including random checks conducted by trained professionals;
e) r\textit{equests for information necessary to \textit{assess} the cybersecurity risk-management measures} adopted by \underline{the entity} concerned, including documented cybersecurity policies, as well as compliance with the obligation to submit information to the \underline{competent authorities} pursuant to Article 27;

Art32(4)  
\underline{Member States} \textbf{shall ensure} that their \underline{competent authorities}, when exercising their enforcement powers in relation to essential entities, have the power at least to: d) order the \underline{entities} concerned to \textit{ensure} that their cybersecurity risk-management \textit{measure}s comply with Article 21 /.../ %or to fulfil the reporting obligations laid down in Article 23
, in a specified manner and within a specified period;
f) order the \underline{entities} concerned to implement the recommendations provided as a result of a security audit within a reasonable deadline;
g) designate a monitoring officer with well-defined tasks \textbf{for a determined period of time to oversee the compliance} of the \underline{entities} concerned with Articles 21 /.../%and Article 23;

Art33(2) 
\underline{Member States} \textbf{shall ensure} that \underline{the competent authorities}, when exercising their supervisory tasks in relation to \underline{important entities}, have the power to subject those entities at least to: a) \textit{on-site inspections and off-site ex post supervision} conducted by \underline{trained professionals}.



\section{Comparison of Security Evaluation Instruments}\label{sec:InstrumentsComparison}
%See jaotis kaob siit ära
\setblue{Vbl on praegune jaotis validationi osas ja siia hoopis see legal textide osa?}
- comparing the instruments, their ability (mentioning in papers) to use them in defined user stories and comparing the previously mentioned criteria.

This section presents an overview of the current state of security evaluation instruments. The reviewed methods are general in nature, meaning they should apply to any organization regardless of size or line of activity. The main focus is determining if these instruments can help entities check if they comply with the NIS2 directive following the defined user stories (see Sec~\ref{sec:UserStoriesDescription}. Also, instruments that rely on technical solutions, like port or vulnerability scanning, are excluded as well if they support NIS2 risk management measures (see Sec~\ref{sec:NIS2}.


This section covers methods proposed in scientific literature and those developed by individual countries (e.g. Kybermittari, Italian Cybersecurity Framework) or inter-governmental agencies (ENISA's EU CSI).

Nations' wish for sovereignty...

Wide range of available tools, but none cover all user stories...

NIS2 does not specify any specific processes or tools to check compliance, only what needs to be covered to be compliant...

Methods introduced in the scientific literature are difficult to implement with the given information...

No immediate feedback, limited feedback, or no feedback at all in some cases...

Due to their methodology, cybersecurity indices do not provide much information on individual organizations...

Notes: What was that Japanese index that gathers info automatically? Add A for automatic into the Format column. Add national audit offices.

Description of criteria used in Table~\ref{tab:RWsummary}:
\begin{itemize}

    \item US1 ...US5 - user stories described in Section \ref{sec:UserStoriesDescription}
    \item NIS2 compliance - the instrument covers all NIS2 requirements for organizations, but also for national offices
    \item Update cycle - how often the instrument is updated
    \item No. of questions - how many aspects are checked with the instrument (may  also show the aggregation level)
    \item Time investment - average time respondents invested on instrument usage
    \item Format - survey, observation, testing, (spreadsheet?) etc.
    \item ISMS coverage - The instrument fully covers some standard requirements (ISO27001, NIST CSF).
    \item Comparability - the results can be compared with other organizations and over time (progress of security implementation).
    \item Entrance barrier - to use the instrument, is there prerequisites to start to use (login, licence fee, introduction work with system, etc.)?
    \item Usable - Is the instrument freely available for use (as a self-assessment tool and does not require one to contact the authors directly)?
    
\end{itemize}


\begin{table}[ht!]
\caption{Summary of security evaluation instruments. '-' means that there is no information provided. '+' means Yes. 'X' means No. In the Format column, S means Survey and P indicates public sources of information}
\label{tab:RWsummary}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.5} % Default value: 1

\begin{tabular}{p{74mm}*{6}{p{4mm}}*{3}{p{9mm}}*{6}{p{4mm}}}
\toprule
\rot{Framework} & \rot{US1} & \rot{US2} & \rot{US3} & \rot{US4} & \rot{US5} & \rot{NIS2 Compliance} & \rot{ISMS coverage} \\

\midrule
F4SLE &  + &  + &  + &  + &  + &  + &    +  \\
\cite{qiangmin2007method} & X &  X &  X &  + &  X &  - &   X   \\
\cite{jazri2018measuring} &  X &  + &  X &  + &  + &  + & \\
\cite{you2016advanced} & X &  X &  X &  + &  + &  + &   X \\
\cite{bernik2016measuring}, \cite{prislan2020real} & X & X  &  + &  + &  + &  + &   &   \\
\cite{maleh2017towards} &  X &  X &  + &  + &  + &  + &  +  \\
\cite{rae2019defining} &  X &  X  &  + &  + &  + &  + &  X \\
\cite{malaivongs2022cybertrust} &  X &  X & + & + & + & + &  X \\
Statistics Boards & + & X & X & X & X & X & X \\
NUKIB report & + & + & X & X &   X &   -  &   - \\
Austrian Information Security Guide \cite{AustriaHandbook} &  &  &  &  &  &    &  \\
Italian Cybersecurity Framework \cite{ITALY} & X & + & + & + & + & -  & - \\
Greek Cybersecurity Self-assessment tool \cite{greeceSelfAssessment} & X & X & + & + & X & X  & X \\
Irish Cybersecurity Baseline Standards Self-assessment tool \cite{irelandSelfAssessment} & X & X & + & + & + & X &  \\
Spanish National Cybersecurity Institute's Self-Assessment Tool \cite{spainSelfAssessment} & X & X & X & + & X & X & X \\
Swiss Cybersecurity QuickCheck \cite{SwitzerlandQuickcheck} &  &  &  &  &  &    &  \\
Kybermittari \cite{KybermittariWeb} & X & + & + & + & + & - & - \\
EU CSI \cite{EUCSI} & + & X & X & X & X & X & X \\ 
NCSI \cite{NCSIWeb} & + & X &  X & X  & X & X & X \\
GCI \cite{GCIWeb} & + & X & X & X & X & X & X \\
NCPI \cite{BelferCent2020NCPI} & + & X & X & X & X & X & X \\
CDI &  &  &  &  &  &   &  \\
O-ISM3 \cite{oism3} & X  & X & X & + & + & X & + \\ 
ISFAM \cite{spruit2014isfam}, \cite{spruit2017isfam} & X & X & X & + & X & - & -  \\
IASME Cyber Essentials \cite{IASMEEssentials} & X  & X & X & + & X & - & - \\ 
C2M2 \cite{C2M2Tool} & X & X & + & + & + & X  & + \\
CIS 20 & X & X & + & + & + & X  & +\\
CMMC & X & X & X & + & X & X & X \\
%NIST-CSF & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ?\\
%ISO 27001 & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ? & ?\\
ENISA NCAF \cite{ENISANCAF} & + & X & X & X & X &  &  \\
ENISA Cybersecurity Maturity Assessment for SMEs \cite{ENISAAssessmentSMEs} &  &  &  &  &  &  &  \\
\bottomrule
\end{tabular}
\end{table}




\subsection{US1: Member State}\label{sec:US_MS}
\begin{itemize}
    \item User role: Member State 
    \item Problem to solve: factual proof of achieving a high common level of cybersecurity in all sectors and entities to avoid cyber incidents caused major damage on economics and society.
    \item Reference: NIS2 Art1(1); Art7(2); Art19(1.a); Art20(1),(2); Art21(1),(2),(3),(4) 
    \begin{itemize}
        \item[US1.1] As a Member State, I can ensure the effective management of cybersecurity risk-management measures in (essential and important) entities by evaluating their security level so that compliance with regulations is achieved.
        \item[US1.2] As a Member State, I can evaluate an entity’s cybersecurity level using an all-hazards approach so that the allocation of resources is addressed directly on identified vulnerabilities.
    \end{itemize}
\end{itemize}

management= implementation, oversight, and improvement
\subsection{US2: Supervisory Authority} \label{sec:US_Supervisory}

\begin{itemize}

    \item User role: Supervisory Authority
    \item Problem to solve: The Supervisory Authority should base on risk assessments when planning their supervisory tasks, but they should optimise the workflow and not unnecessarily hamper the business activities of the entity concerned.
    \item Reference: Art21(1),(2),(4); Art31(2); Art32(2); Art32(4); Art33(2)

    \begin{itemize}
        \item[US2.1] As a Supervisory Authority, I can prioritise supervisory tasks by using all hazard-covering security evaluation results so that supervisory tasks focus on high-risk entities or areas.
        \item[US2.2] As a Supervisory Authority, I can ensure with a remote security evaluation that entities that did not comply with regulatory requirements implement corrective risk-management measures within reasonable deadlines so that supervisory resources are used effectively and unnecessarily hamper the business activities of the entity is avoided.
    \end{itemize}
\end{itemize}

\subsection{US3: ENISA}\label{sec:US_ENISA}
\begin{itemize}
    \item User role: ENISA
    \item Problem to solve: collect data to evaluate EU security level and report the result to EU Parliament
    \item Reference: NIS2 Art1(1), Art18(1)
    \begin{itemize}
        \item[US3.1] As ENISA, I can collaborate with Member States to assess collected evaluation data on cybersecurity capabilities and awareness so that identifying the cybersecurity gaps enables enhanced cybersecurity practices across the European Union.
    \end{itemize}
\end{itemize}


\subsection{US4: Security Consultant}\label{sec:US_Consultant}
\begin{itemize}
    \item User role: Security Consultant
    \item Problem to solve: Consultants should help improve the entity's security level by finding and focusing on vulnerable areas of the entity. 
    \item Requirements/needs: Art20(2); Art21(2) 

    \begin{itemize}
        \item[US4.1] As a security consultant, I can get an overview of the entity's security maturity evaluation results so that the most vulnerable areas can be prioritized in a timely manner for an improvement plan.
        \item[US4.2] As a security consultant, I can re-evaluate the entity's risk management measures implementation so that tracking characterises risk management measures implementation status progress.
    \end{itemize}
\end{itemize}

\subsection{US5: Entity }\label{sec:US_Entity}
\begin{itemize}
    \item User role: Members of the Management Bodies 
    \item Problem to solve: to obtain an overview of the entity's cybersecurity risk management measures all-hazard approach to confirm security status and improve vulnerable areas 
    \item Requirements/needs: Art20(2); Art21(2)
    \begin{itemize}
        \item[US5.1]As an entity, I can ensure the entity adopts an all-hazards approach to cybersecurity so that the evaluation results show strengths and direct to plan improvements to our security shortcomings.   
        
    \end{itemize}
\end{itemize}

\subsection{US6: Service Provider \& Supplier}\label{sec:US_Supplier}
\begin{itemize}
    \item User role: Service Provider \&  Supplier 
    \item Problem to solve: get an evaluation of Service Provider \&  Supplier security to share with partners and assess compliance with partner requirements
    \item Requirements/needs: Art21(2); Art21(3)

    \begin{itemize}
        \item[US6.1]  As a Service Provider \&  Supplier, I can provide the risk management measures in all-hazard evaluation approach results to the partner Entity so that the Entity can choose the most (suitable) secure suppliers.
        \item[US6.2]   As a Service Provider \&  Supplier, I can regularly evaluate my cybersecurity practices so that my partner Entity can get a sense of security in the supply chain.
    \end{itemize}
\end{itemize}


%=====================================
European Commission NIS2 Directive \cite{NIS2} aims to increase overall cybersecurity capabilities throughout the European Union, reduce risks and enable the operation of critical and important services in the event of incidents so that the economy and society can continue to function sustainably.
For society to function, in addition to the tasks of state or EU-level management bodies like CSIRT, cooperation groups, or others, risk management measures must be ensured in specific organizations of essential and important service providers. Based on the minimal requirements provided by NIS2, member states (MS) determine the national security requirements for organizations (Art 5 of \cite{NIS2}). 

Organizations applying NIS2 must create the capability to report incidents, i.e. establish an incident management procedure (Art23 of \cite{NIS2}). Still, they must also follow the required training for management bodies and their employees (Art20 of \cite{NIS2}).

Additionally are required technical, operational and organizational risk management measures (NIS2 Art21(2)). %like \textit{(a)} policies on risk analysis and information system security, \textit{(b)} incident handling, \textit{(c)} business continuity (backups, recovery and crisis management), \textit{(d)} supply chain security, \textit{(e)} network and system acquisition, development and maintenance, \textit{(f)} ISMS effectiveness assessment measures, \textit{(g)} cyber-hygiene and training, \textit{(h) }usage of cryptography and encryption, \textit{(i)} human resources security, including access and asset management, \textit{(j)} use of multi-factor authentication and secure media and communication resources. \cite{NIS2}
NIS2 requires organizations' risk management measures but defines them at a high general level, and organizations with low cybersecurity maturity levels need additional implementation support from consultants and government bodies.

Art31-33 of NIS2 \cite{NIS2} stipulates that national supervisory authorities evaluate organizations' adherence to the prescribed risk management measures. As the number of organizations mandated to implement NIS2 risk management measures rises sharply, supervisory bodies must also adjust to enhance their visibility and efficacy.

Art19 of NIS2 \cite{NIS2} states that in evaluating the level of cyber security, the MS can voluntarily participate through a peer review procedure organized by the  Cooperation Group, during which the implementation of the risk management measures described in Art21 and Art23 is evaluated.

NIS2 leaves the assessment of overall high-security level in member state organizations open. The directive uses keywords such as \textit{ensure}, \textit{oversee}, \textit{assess} but does not put them in a format that explains the nature of the measurement or evaluation method.
However, the methods of obtaining factual confirmation are measurements, evaluations or assessments based on data collection and comparison with the past \setblue{TODO CITE?}, which directly indicates the need for security evaluation.
There are several security evaluation instruments \setblue{TODO CITE?}, but few studies evaluate how well these instruments comply with NIS2 requirements\setblue{TODO CITE?}. 
By defining user stories consistent with the goals of NIS2, existing security evaluation instruments could be adapted and improved, or new ones could be designed consistently from scratch.
%====================

%The supervisory and enforcement regimes for those two categories of entities should be differentiated to ensure a fair balance between risk-based requirements and obligations on the one hand, and the administrative burden stemming from the supervision of compliance on the other.[15)]

%Furthermore, in order to streamline supervisory activities between the competent authorities under this Directive and those under Directive (EU) 2022/2557 and in order to minimise the administrative burden for the entities concerned, those competent authorities should endeavour to harmonise incident notification templates and supervisory processes.[30]

%entities should evaluate their own cybersecurity capabilities and, where appropriate, pursue the integration of cybersecurity enhancing technologies, such as artificial intelligence or machine-learning systems to enhance their capabilities and the security of network and information systems.[89]

% essential entities should be subject to a comprehensive ex ante and ex post supervisory regime, while important entities should be subject to a light, ex post only, supervisory regime.[122] 

% The execution of supervisory tasks by the competent authorities should not unnecessarily hamper the business activities of the entity concerned. Where the competent authorities execute their supervisory tasks in relation to essential entities, including the conduct of on-site inspections and off-site supervision, the investigation of infringements of this Directive and the conduct of security audits or security scans, they should minimise the impact on the business activities of the entity concerned.[123]

%Supervisory tasks should minimise the impact on business activities of essential services.
%Supervisory tasks prioritization should include criteria or benchmarks for the classification of essential entities into risk categories [124]

